Null-text Inversion for Editing Real Images using Guided Diffusion Models

Recent text-guided diffusion models provide powerful image generation capabilities. Currently, a massive effort is given to enable the modification of these images using text only as means to offer intuitive and versatile editing. To edit a real image using these state-of-the-art tools, one must first invert the image with a meaningful text prompt into the pretrained model's domain. In this paper, we introduce an accurate inversion technique and thus facilitate an intuitive text-based modification of the image. Our proposed inversion consists of two novel key components: (i) Pivotal inversion for diffusion models. While current methods aim at mapping random noise samples to a single input image, we use a single pivotal noise vector for each timestamp and optimize around it. We demonstrate that a direct inversion is inadequate on its own, but does provide a good anchor for our optimization. (ii) NULL-text optimization, where we only modify the unconditional textual embedding that is used for classifier-free guidance, rather than the input text embedding. This allows for keeping both the model weights and the conditional embedding intact and hence enables applying prompt-based editing while avoiding the cumbersome tuning of the model's weights. Our Null-text inversion, based on the publicly available Stable Diffusion model, is extensively evaluated on a variety of images and prompt editing, showing high-fidelity editing of real images.

==> figures/comparison_ablation.tex <==
\begin{figure*}[t]
\centering 
\includegraphics[width=\textwidth]{figures/comparison_ablation2.pdf} 

\vspace{-0.2cm}
\caption{Qualitative comparison for the ablation study showing the inversion results after $200$ optimizations iterations of our full algorithm (on right) compared to other baselines. Full figure with for all iterations is shown in the supplementary.} \vspace{-0.5cm}
\label{fig:exp_ablation_qual} 

\end{figure*}


==> figures/experiments_graph_sdedit.tex <==
\begin{figure}[t]
\centering 
\includegraphics[width=\columnwidth]{figures/experiments_graph_sdedit_pdf.pdf} 
% \vspace{-0.3cm}
\caption{Editing evaluation using SDEdit with and without our method. Applying SDEdit with NULL- Text embedding better preserves fidelity with respect to the input image (low LPIPS score) while aligning to the edit text (high CLIPscore).} 
\label{fig:exp_graph_sdedit} 
\vspace{-0.3cm}
\end{figure}


==> sup_figures/comparison_sup2.tex <==
\begin{figure*}
% \setlength{\belowcaptionskip}{-12pt}
% \setlength{\abovecaptionskip}{2.0pt}
\setlength{\tabcolsep}{2.0pt}
    \centering
    { %\scriptsize %\footnotesize

\begin{tabular}{c | c c c c c}


\multicolumn{1}{c}{{ \bf Input}}&
\multicolumn{1}{c}{{ \bf Our Inversion}}&
\multicolumn{1}{c}{{ \bf Text2LIVE}}&
\multicolumn{1}{c}{{ \bf VQGAN+CLIP}}&
\multicolumn{1}{c}{{ \bf SDEdit}}&
\multicolumn{1}{c}{{ \bf Our Editing}} \\














{\includegraphics[width=0.16\textwidth]{images/gt/034.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/inversion/waterfall.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/text2live/waterfall_034.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/vqclip/034.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/sde/waterfall_034.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/ours/waterfall_034.jpg}} \\



 & \multicolumn{5}{c}{"a bridge over a {\color{RoyalPurple} \bf frozen} waterfall"} \\
 &&& \\


{\includegraphics[width=0.16\textwidth]{images/gt/034.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/inversion/waterfall.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/text2live/waterfall_038.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/vqclip/038.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/sde/waterfall_038.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/ours/waterfall_038.jpg}} \\



 & \multicolumn{5}{c}{"A {\color{RoyalPurple} \bf golden} bridge over a waterfall"} \\
 &&& \\


% {\includegraphics[width=0.16\textwidth]{images/gt/cake_014.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/cake_009.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/009.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/cake_009.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/cake_009.jpg}} \\



% \multicolumn{6}{c}{"A {\color{RoyalPurple} \bf brioche} cake on a table"} \\


% {\includegraphics[width=0.16\textwidth]{images/gt/cake_014.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/inversion/cake_t2l.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/cake_10.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/010.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/cake_010.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/cake_010.jpg}} \\


%  & \multicolumn{5}{c}{"A {\color{RoyalPurple} \bf spinach moss} cake on a table"} \\
%  &&& \\


% {\includegraphics[width=0.16\textwidth]{images/gt/cake_014.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/inversion/cake_t2l.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/cake_15.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/015.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/cake_015.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/cake_015.jpg}} \\



%  & \multicolumn{5}{c}{"A {\color{RoyalPurple} \bf birthday} cake on a table"} \\







\end{tabular}
}


\vspace{-0.2cm}
\caption{{\bf Additional comparison results.}}
\vspace{-0.5cm}
% \vspace{-0.15cm}
% \ron{The gap is best viewed in the supplementary videos.}}
\label{fig:supp_comparison2} %\vspace{-7pt}
\end{figure*}

==> sup_figures/imagic.tex <==
\begin{figure*}
% \setlength{\belowcaptionskip}{-12pt}
% \setlength{\abovecaptionskip}{2.0pt}
\setlength{\tabcolsep}{2.0pt}
    \centering
    { %\scriptsize %\footnotesize

\begin{tabular}{c | c c c c c}


{ \bf Input}&
{ \bf Imagic, $\alpha=0.6$}&
{ \bf Imagic, $\alpha=0.7$}&
{ \bf Imagic, $\alpha=0.8$}&
{ \bf Imagic, $\alpha=0.9$}&
{ \bf Ours} \\





% {\includegraphics[width=0.16\textwidth]{images/gt/034.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/inversion/waterfall.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/waterfall_034.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/034.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/waterfall_034.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/waterfall_034.jpg}} \\



% \multicolumn{6}{c}{"a bridge over a {\color{RoyalPurple} \bf frozen} waterfall"} \\



% {\includegraphics[width=0.16\textwidth]{images/gt/034.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/inversion/waterfall.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/waterfall_038.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/038.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/waterfall_038.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/waterfall_038.jpg}} \\



% \multicolumn{6}{c}{"A {\color{RoyalPurple} \bf golden} bridge over a waterfall"} \\



% % {\includegraphics[width=0.16\textwidth]{images/gt/cake_014.jpg}}&
% % {\includegraphics[width=0.16\textwidth]{images/text2live/cake_009.jpg}} &
% % {\includegraphics[width=0.16\textwidth]{images/vqclip/009.jpg}} &
% % {\includegraphics[width=0.16\textwidth]{images/sde/cake_009.jpg}} &
% % {\includegraphics[width=0.16\textwidth]{images/ours/cake_009.jpg}} \\



% % \multicolumn{6}{c}{"A {\color{RoyalPurple} \bf brioche} cake on a table"} \\


% {\includegraphics[width=0.16\textwidth]{images/gt/cake_014.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/inversion/cake_t2l.jpg}}&
% {\includegraphics[width=0.16\textwidth]{images/text2live/cake_10.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/vqclip/010.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/sde/cake_010.jpg}} &
% {\includegraphics[width=0.16\textwidth]{images/ours/cake_010.jpg}} \\



% \multicolumn{6}{c}{"A {\color{RoyalPurple} \bf spinach moss} cake on a table"} \\


{\includegraphics[width=0.16\textwidth]{images/gt/135.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/134_6.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/134_7.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/134_8.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/134_9.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/ours/aviv_134.jpg}} \\



 & \multicolumn{5}{c}{"A baby holding her \st{monkey} {\color{RoyalPurple} \bf lion} doll"} \\



{\includegraphics[width=0.16\textwidth]{images/gt/153.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/147_6.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/147_7.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/147_8.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/147_9.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/ours/cake_147.jpg}} \\



 & \multicolumn{5}{c}{"A {\color{RoyalPurple} \bf spinach moss} cake on a table"} \\


{\includegraphics[width=0.16\textwidth]{images/gt/159.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/166_6.jpg}}&
{\includegraphics[width=0.16\textwidth]{images/imagic/166_7.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/166_8.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/imagic/166_9.jpg}} &
{\includegraphics[width=0.16\textwidth]{images/ours/cake_166.jpg}} \\



 & \multicolumn{5}{c}{"A piece of {\color{RoyalPurple} \bf unicorn} cake"} \\





\end{tabular}
}


\vspace{-0.2cm}
\caption{{\bf Comparison to Imagic \cite{Kawar2022ImagicTR}. {\it We employ the unofficial Imagic implementation for Stable Diffusion and present the results for different values of the interpolation parameter $\alpha$, which is used to interpolate between the target text embedding and the optimized one \cite{Kawar2022ImagicTR}, where increasing $\alpha$ increases the fidelity to the target text. As can be seen, Imagic struggles to preserve the original details, such as the identity of the baby ($1$st row) or cups in the background ($2$nd row). In addition, we observe that each example requires a separate tuning of the $\alpha$ parameter.} }}
\vspace{-0.5cm}
% \vspace{-0.15cm}
% \ron{The gap is best viewed in the supplementary videos.}}
\label{fig:imagic} %\vspace{-7pt}
\end{figure*}
